A Mechanized Proof of Bounded Convergence Time for the Distributed Perimeter Surveillance System (DPSS) Algorithm A

The decentralized perimeter surveillance system (DPSS) seeks to provide a decentralized protocol for evenly distributing surveillance of a perimeter over time across an ensemble of unmanned aerial vehicles (UAVs) whose members may communicate only when in close proximity to each other. The protocol must also converge to an even distribution of the perimeter in bounded time. Two versions of the DPSS protocol presented in the original paper seem to converge in bounded time but only informal proofs and arguments are given. A later application of model checking to these protocols found an error in one of the key lemmas, invalidating the informal proof for one and casting doubt on the other. Therefore, a new hand proof of the convergence time for the simpler version of the DPSS protocol or algorithm, Algorithm A or DPSS-A, was developed by Jeremy Avigad and Floris van Doorn. This paper describes a mechanization of that hand proof in the logic of ACL2 and discusses three specific ACL2 utilities that proved useful for expressing and reasoning about the DPSS model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{33}
\providecommand{\publicationstatus}{Rob Sumners, Cuong Chau (Eds.): 17th ACL2 Workshop (ACL2 2022)\\
EPTCS 359, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.359.5}{10.4204/EPTCS.359.5}}

